Supportive Fintech for Individuals with Bipolar Disorder: Financial Data Sharing Preferences to Support Longitudinal Care Management

Financial stability is a key challenge for individuals living with bipolar disorder (BD). Symptomatic periods in BD are associated with poor financial decision-making, contributing to a negative cycle of worsening symptoms and an increased risk of bankruptcy. There has been an increased focus on designing supportive financial technologies (fintech) to address varying and intermittent needs across different stages of BD. However, little is known about this population's expectations and privacy preferences related to financial data sharing for longitudinal care management. To address this knowledge gap, we have deployed a factorial vignette survey using the Contextual Integrity framework. Our data from individuals with BD (N=480) shows that they are open to sharing financial data for long term care management. We have also identified significant differences in sharing preferences across age, gender, and diagnostic subtype. We discuss the implications of these findings in designing equitable fintech to support this marginalized community.

==> tables/overall-ratings.tex <==
\hypertarget{tbl-overall}{}
\begin{longtable}[]{@{}lrrrr@{}}
\caption{\label{tbl-overall}Participants were most comfortable sharing
financial data when they were the recipient of insights delivered by the
hypothetical application.}\tabularnewline
\toprule\noalign{}
\textbf{Recipient} & \textbf{Mean} & \textbf{Median} & \textbf{SD} &
\textbf{Obs} \\
\midrule\noalign{}
\endfirsthead
\toprule\noalign{}
\textbf{Recipient} & \textbf{Mean} & \textbf{Median} & \textbf{SD} &
\textbf{Obs} \\
\midrule\noalign{}
\endhead
\bottomrule\noalign{}
\endlastfoot
Clinician & 5.57 & 6 & 3.03 & 1732 \\
Family & 5.00 & 5 & 3.08 & 1807 \\
Self & 7.56 & 8 & 2.66 & 1492 \\
\end{longtable}
